Learning to Drive in a Day

We demonstrate the first application of deep reinforcement learning to autonomous driving. From randomly initialised parameters, our model is able to learn a policy for lane following in a handful of training episodes using a single monocular image as input. We provide a general and easy to obtain reward: the distance travelled by the vehicle without the safety driver taking control. We use a continuous, model-free deep reinforcement learning algorithm, with all exploration and optimisation performed on-vehicle. This demonstrates a new framework for autonomous driving which moves away from reliance on defined logical rules, mapping, and direct supervision. We discuss the challenges and opportunities to scale this approach to a broader range of autonomous driving tasks.

==> figures/task-diagram.tex <==

\begin{figure}
\centering
\resizebox{5cm}{!}{%
    \tikzstyle{block} = [rectangle, draw, text width=8em, text centered,
    rounded corners, minimum height=3em]
    \begin{tikzpicture}[align = center, node distance = 8em, auto, thick]
        \node [block] (Trainer) {Trainer};
        \node [block, below of=Trainer, yshift=+0.5cm] (Model) {Model};
        \node [block, below of=Model, yshift=+0.5cm] (Controller) {Controller};
        \node [block, below of=Controller, yshift=+0.5cm] (Vehicle) {Vehicle};

        \node [left of=Model, xshift=0.5cm] (t1) {\includegraphics[width=.05\textwidth]{clock.png}\\10Hz};
        \node [left of=Controller, xshift=0.5cm] (t2)  {\includegraphics[width=.05\textwidth]{clock.png}\\100Hz};

        \coordinate [right of=Model, xshift=0.5cm] (t1);
        \coordinate [right of=Controller, xshift=0.5cm] (t2);
        \coordinate [right of=Vehicle, xshift=0.5cm] (t3);

        \draw [-{Latex[width=2mm]}] (Trainer) -- (Model);
        \draw [-{Latex[width=2mm]}] (Model) edge node[right] {Speed, Steering} (Controller);
        \draw [-{Latex[width=2mm]}] (Controller) -- (Vehicle);
        \draw [-{Latex[width=2mm]}] (t1) -- node[above] {Image +} node[below] {Steering} (Model);
        \draw [-{Latex[width=2mm]}] (t2) -- (Controller);
        \draw [-] (t3) -- (Vehicle);
        \draw [-] (t1) -- (t3);
    \end{tikzpicture}
}
\caption{Policy execution architecture, used to run episodes during model training (or run continuously under test).}
\label{fig:rl-training-logic}
\end{figure}

